On Construction of a Class of Orthogonal Arrays (Thesis)

We propose a novel method for the construction of orthogonal arrays. The algorithm makes use of the Kronecker Product operator in association with unit column vectors to generate new orthogonal arrays from existing orthogonal arrays. The effectiveness of the proposed algorithm lies in the fact that it works well with any linear seed orthogonal array without imposing any constraints on the strength or the number of levels. The resulting orthogonal array has the same strength as the seed orthogonal array. We also discuss the proof of correctness of the algorithm. In the Results section we provide a list of new orthogonal arrays generated using this algorithm, that are currently not present in the libraries of orthogonal arrays.

==> chapter-futurework.tex <==
\chapter{Future Work\label{ch:futurework}}
Future work should include options in the template for a masters thesis or an undergraduate senior thesis. It should also support running headings in the headers using the `headings' pagestyle.  The print mode and proquest mode included in the template might also be candidates to include in the class itself. 

 

==> references.tex <==
\begin{enumerate}
\item Hedayat, A. , Sloane, N.J.A. and Stufken, J. (1999).Orthogonal Arrays. \textit{Springer-Verlag}, New York.\\
\item Shrikhande, S.S. (1964). Generalised Hadamard matrices and orthogonal arrays of strength two. \textit{Canadian J. Math}, \textbf{16}, 736-740. \\
\item Wang, J. C. and Wu, C. F. J. (1991). An approach to construction of asymmetrical orthogonal arrays. \textit{J. Amer. Statist. Assoc.}, \textbf{86}, 450-456. \\
\item Zhang, Y., Weiguo, L., Mao, S., Zheng, Z. (2006). A simple method for constructing orthogonal arrays by the Kronecker sum. \textit{J. Syst. Sci. Complexity}, \textbf{19}, 266-273. \\
\item Sinha, K., Vellaisamy, P., Sinha, N. (2008). Kronecker sum of binary orthogonal arrays. \textit{Utilitas Mathematica,} \textbf{75}, 249-257.\\
%\item Sinha, K., Kumar, S., Sen Gupta, A. (2009). Construction of ternary orthogonal arrays by Kronecker sum. \textit{J. Stat. & Appl.} \textbf{Vol. 4}, No. 2-3, 2009, pages 475-47. \\
\item Sinha, K., Mathur, S. N. and Nigam, A. K. (1979). Kronecker sum of incomplete block designs. \textit{Utilitas Mathematica}, \textbf{16}, 157-164.
\end{enumerate}
